An Initial Exploration: Learning to Generate Realistic Audio for Silent Video

Generating realistic audio effects for movies and other media is a challenging task that is accomplished today primarily through physical techniques known as Foley art. Foley artists create sounds with common objects (e.g., boxing gloves, broken glass) in time with video as it is playing to generate captivating audio tracks. In this work, we aim to develop a deep-learning based framework that does much the same - observes video in it's natural sequence and generates realistic audio to accompany it. Notably, we have reason to believe this is achievable due to advancements in realistic audio generation techniques conditioned on other inputs (e.g., Wavenet conditioned on text). We explore several different model architectures to accomplish this task that process both previously-generated audio and video context. These include deep-fusion CNN, dilated Wavenet CNN with visual context, and transformer-based architectures. We find that the transformer-based architecture yields the most promising results, matching low-frequencies to visual patterns effectively, but failing to generate more nuanced waveforms.

==> bib_commands.tex <==
****** Note: this is not a real tex document. I just gave it the extension so that you'd get tex-style syntax highlighting ******

Rather than using the bibitem package, as the IEEE sample does, I recommend using BibTex. Copy the bibliography folder into the folder containing your main document. Before the \begin{document}, you should include

\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

At the end of your file, before the \end{document}, you should include

\bibliographystyle{./bibliography/IEEEtran}
\bibliography{./bibliography/IEEEabrv,./bibliography/references}

All your citations should go inside \verb=/bibliography/references.bib=. Remember that you can usually download a BibTex citation for any resource you use from Google Scholar or Arxiv, and just copy it into \verb=references.bib=. 



